Artificial Intelligence and Strategic Decision-Making: Evidence from Entrepreneurs and Investors

This paper explores how artificial intelligence (AI) may impact the strategic decision-making (SDM) process in firms. We illustrate how AI could augment existing SDM tools and provide empirical evidence from a leading accelerator program and a startup competition that current Large Language Models (LLMs) can generate and evaluate strategies at a level comparable to entrepreneurs and investors. We then examine implications for key cognitive processes underlying SDM -- search, representation, and aggregation. Our analysis suggests AI has the potential to enhance the speed, quality, and scale of strategic analysis, while also enabling new approaches like virtual strategy simulations. However, the ultimate impact on firm performance will depend on competitive dynamics as AI capabilities progress. We propose a framework connecting AI use in SDM to firm outcomes and discuss how AI may reshape sources of competitive advantage. We conclude by considering how AI could both support and challenge core tenets of the theory-based view of strategy. Overall, our work maps out an emerging research frontier at the intersection of AI and strategy.

==> figs/descrip-stats-eval.tex <==
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{5}{ccccccc}}
\hline\hline
                    &\multicolumn{1}{c}{Mean}&\multicolumn{1}{c}{SD}&\multicolumn{1}{c}{ Min.}&\multicolumn{1}{c}{Max.}&\multicolumn{1}{c}{Count}\\
                    &            &            &            &            &            \\
\hline
Years of investment experience&        4.85&        4.85&        0.00&       30.00&         100\\
Number of investments&        3.71&        6.65&        0.00&       50.00&         100\\
Experience - angel investing&        0.40&        0.49&        0.00&        1.00&         100\\
Experience - venture capital&        0.71&        0.46&        0.00&        1.00&         100\\
Experience - private equity&        0.00&        0.00&        0.00&        0.00&         100\\
Years of work experience&       18.11&        9.15&        3.00&       30.00&         100\\
Years of managerial experience&        8.63&        7.85&        0.00&       30.00&         100\\
Degree higher than college&        0.22&        0.42&        0.00&        1.00&         100\\
Female              &        0.26&        0.44&        0.00&        1.00&         100\\
\hline\hline
\end{tabular}

